Working Paper: Conflicts and the New Scramble for African Resources -- A Shift-Share Approach

This paper estimates the causal effect of mineral trade on conflicts in Africa using a Shift-Share IV approach based on an exogenous price-commodity shock. The main result is that an increase in mineral trade significantly increases the number of conflicts while it has no clear effect on fatalities. Exploring heterogeneous effects, I find that a specific group of minerals, oil and fuels, drives the results on the number of conflicts. Moreover, the group of rare minerals such as coltan, precious metals or cobalt has no effect on the number of conflicts but appears to have an important impact on the number of fatalities.

==> Falsification.tex <==
\begin{table}[htbp]\centering
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Falsification Test }
\begin{tabular}{l*{4}{c}}
\hline\hline
            &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}\\
            &\multicolumn{1}{c}{lagged1\_number\_conflict}&\multicolumn{1}{c}{lagged2\_number\_conflict}&\multicolumn{1}{c}{lagged1\_fatalities}&\multicolumn{1}{c}{lagged2\_fatalities}\\
\hline
normalized\_mineral\_value&       0.009   &       0.010   &      -0.111***&       0.051   \\
            &     (0.015)   &     (0.016)   &     (0.043)   &     (0.132)   \\
\hline
F\_test\_     &   30858.596   &    9198.324   &   30858.596   &    9198.324   \\
\hline\hline
\multicolumn{5}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{5}{l}{\footnotesize * p<.1, ** p<.05, *** p<.01}\\
\end{tabular}
\end{table}


==> Falsification_a.tex <==
\begin{table}[htbp]\centering
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Falsification Test a}
\begin{tabular}{l*{4}{c}}
\hline\hline
            &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}\\
            &\multicolumn{1}{c}{log\_lag\_1\_conflict}&\multicolumn{1}{c}{log\_lag\_1\_conflict}&\multicolumn{1}{c}{log\_lag\_1\_fatalities}&\multicolumn{1}{c}{log\_lag\_1\_fatalities}\\
\hline
log\_x\_mineral&       0.537** &       0.168   &       0.273   &       0.107   \\
            &     (0.252)   &     (0.149)   &     (0.275)   &     (0.230)   \\
\hline
F\_test\_     &      10.922   &      16.222   &       9.173   &      12.630   \\
\hline\hline
\multicolumn{5}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{5}{l}{\footnotesize * p<.1, ** p<.05, *** p<.01}\\
\end{tabular}
\end{table}


==> Heterogeneity_tab.tex <==
\begin{table}[htbp]\centering
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Heterogeneity Results}
\begin{tabular}{l*{4}{c}}
\hline\hline
            &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}\\
            &\multicolumn{1}{c}{number\_conflict}&\multicolumn{1}{c}{number\_conflict}&\multicolumn{1}{c}{fatalities}&\multicolumn{1}{c}{fatalities}\\
\hline
normalized\_mineral\_value\_25&      -0.461   &      -0.461   &       2.360***&       2.360   \\
            &     (0.418)   &     (0.913)   &     (0.719)   &     (1.534)   \\
[1em]
normalized\_mineral\_value\_26&      -0.098   &      -0.098   &       0.362***&       0.362*  \\
            &     (0.069)   &     (0.125)   &     (0.119)   &     (0.201)   \\
[1em]
normalized\_mineral\_value\_27&       0.064***&       0.064*  &      -0.110***&      -0.110*  \\
            &     (0.012)   &     (0.034)   &     (0.020)   &     (0.056)   \\
[1em]
normalized\_non\_mineral\_value&      -0.224***&      -0.224** &       0.042   &       0.042   \\
            &     (0.052)   &     (0.106)   &     (0.089)   &     (0.142)   \\
\hline
F\_test\_     &     186.598   &           .   &     186.598   &           .   \\
\hline\hline
\multicolumn{5}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{5}{l}{\footnotesize * p<.1, ** p<.05, *** p<.01}\\
\end{tabular}
\end{table}


==> RQ_and_motivation.tex <==
\section{Introduction}

\begin{comment}
\textbf{Research question:} how does mineral trade impact conflict in Africa? \\

\noindent \textbf{Motivation:} A select group of  minerals and elements that are vital for energy and battery technologies are also likely to undergo rapid increases in demand as a result of the move toward low- and zero-CO2 energy and transportation technology driven by climate change mitigation and consumer and investor concerns and demands \citep{jowitt2021battery}. Hence, evaluating the social cost of this increase in demand is paramount. 
\end{comment}

\begin{comment}
    

Civil wars and violent conflicts have proliferated in Africa over the last decades. Between 1960 and 2000, close to 20 African nations encountered at least one episode of civil war \citep{elbadawi2000there}. During the mid-1990s, about one in three sub-Saharan African country had active civil wars or conflicts \citep{blattman2010civil}. Literature has shown that mining activity increases the incidence of conflicts at the local level subsequently disseminating violence across broader territories \citep{berman2017mine, de2020origin}. In a changing world where a critical subset of minerals and elements essential for energy and battery technologies is likely to experience rapid growth in demand due to the shift toward CO2-neutral policies,\citep{jowitt2021battery}, evaluating the social cost (coming from conflicts) of this increase in demand is paramount. \\



\noindent To measure such a social cost, this paper investigates the impact of mineral trade on conflict in Africa between 2000 and 2020 using a SSIV methodology based on an exogenous price-commodity shock weighted by mineral industry shares reflecting heterogeneous shock exposure \citep{borusyak2022quasi}. From an economic theory perspective, the hypothesis tested here is that an increase in demand for minerals from the global market because of several factors (climate change related or not) increases conflict through higher incentives to fight for scarce resources. An additional question of interest is to know whether existing conflicts become more fatal if the stakes are higher.  \\

\noindent The contribution of this study is twofold. First, applying a SSIV methodology for the first time in this context enables to evaluate whether the pretty well-established result that an increase in natural resources trade increases conflict is robust to this method. Most importantly, the structure of the data allows to investigate which type of mineral trade matters for two conflict indicators (number of conflicts and fatalities), which provides policy relevant information, notably in the context of climate change. Indeed, this study aims at providing a comprehensive and systematic presentation of which type of mineral matters for conflict in Africa, a question that has not been extensively covered in the literature. Understanding which minerals play critical roles in the stability of resource-rich nations could serve as an additional factor to consider when designing future environmental policies. \\

\noindent Matching trade data at the country level (UN Comtrade) and conflict data from the Armed Conflict Location Events Data (ACLED), I find that an increase in mineral trade has a causal effect on the number of conflicts but not on number of fatalities. This result is robust to different specifications and falsification tests. When it comes to which type of minerals matters, it seems that only mineral fuels/oils such as gas or
petrol matter for the number of conflicts. Moreover, rare minerals such as coltan, precious metals or cobalt have no effect on the number of conflicts but have an important impact on the number of fatalities, potentially  consistent with the hypothesis that
an increase in demand for this type of rare resources leads to an increase in violence and the degree of mortality of conflicts.   \\

\noindent The remainder of this paper is organized as follows. Section 2 presents the political background and Section 3 discusses the data used. Section 4 introduces the methodology and Section 5 the main results. Finally, I present the heterogeneity analysis in Section 6 while  Section 7 concludes. 
\end{comment}

A new type of African natural resources are becoming increasingly valuable in a technology driven world where a critical subset of minerals essential for energy and battery technologies experience rapid growth in demand notably due to the shift toward CO2-neutral policies \citep{jowitt2021battery}. Several external forces therefore compete for such global commodities, creating a new wave of the Scramble for Africa.  \\

\noindent Historically, the 19th century scramble for african resources effectively started with the Berlin Conference (1884-1885) and the partitioning of Africa among European countries. Fragmentation of Africa had long term effects notably on political boundaries \citep{griffiths1986scramble} and on ethnic partitioning, implying higher incidence, severity and duration of political violence \citep{michalopoulos2016long}. Interestingly, this new wave of scramble for Africa involves non-european actors such as America or Asian countries, in particular China \citep{okeke2008second}. This worldwide demand and rising interest for Africa's natural resources raises the stakes and hence potentially conflicts in the region. Literature has shown that mining activity increases the incidence of conflicts at the local level subsequently disseminating violence across broader territories \citep{berman2017mine, de2020origin}. \\  

\noindent To measure the social cost of this new scramble for African minerals, this paper investigates the impact of mineral trade on conflict in Africa between 2000 and 2020 using a SSIV methodology based on an exogenous price-commodity shock weighted by mineral industry shares reflecting heterogeneous shock exposure \citep{borusyak2022quasi}. From an economic theory perspective, the hypothesis investigated is that higher demand for minerals from the global market because of several factors (climate change related or not) increases conflict through higher incentives to fight and scramble for scarce resources. An additional question of interest is to know whether existing conflicts become more fatal if the stakes are higher.  \\

\noindent The contribution of this study is twofold. First, applying a SSIV methodology for the first time in this context enables to evaluate whether the pretty well-established result that a rise in natural resources trade increases conflict is robust to this method. Most importantly, the structure of the data allows to investigate which type of mineral trade matters for two conflict indicators (number of conflicts and fatalities), which provides policy relevant information, notably in the context of climate change. Indeed, this study aims at providing a comprehensive and systematic presentation of which type of mineral matters for conflict in Africa, a question that has not been extensively covered in the literature. Understanding which minerals play critical roles in the stability of resource-rich nations could serve as an additional factor to consider when designing future environmental policies. \\

\noindent Matching trade data at the country level (UN Comtrade) and conflict data from the Armed Conflict Location Events Data (ACLED), I find that higher mineral trade has a causal effect on the number of conflicts but not on number of fatalities. This result is robust to different specifications and falsification tests. When it comes to which type of minerals matters, it seems that only mineral fuels/oils such as gas or
petrol matter for the number of conflicts. Moreover, rare minerals such as coltan, precious metals or cobalt have no effect on the number of conflicts but have an important impact on the number of fatalities, potentially  consistent with the hypothesis that
growing demand for this type of rare resources leads to an escalation in violence and the degree of mortality of conflicts.   \\

\noindent The remainder of this paper is organized as follows. Section 2 presents the political background and Section 3 discusses the data used. Section 4 introduces the methodology and Section 5 the main results. Finally, I present the heterogeneity analysis in Section 6, highlight some limitations in section 7  while  Section 8 concludes. 


==> Results_a.tex <==
\begin{table}[htbp]\centering
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Main Results}
\begin{tabular}{l*{6}{c}}
\hline\hline
            &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}\\
            &\multicolumn{1}{c}{number\_conflict}&\multicolumn{1}{c}{number\_conflict}&\multicolumn{1}{c}{number\_conflict}&\multicolumn{1}{c}{fatalities}&\multicolumn{1}{c}{fatalities}&\multicolumn{1}{c}{fatalities}\\
\hline
normalized\_mineral\_value&       0.007** &       0.059***&       0.059*  &       0.015   &      -0.078***&      -0.059   \\
            &     (0.003)   &     (0.012)   &     (0.033)   &     (0.017)   &     (0.015)   &     (0.048)   \\
[1em]
normalized\_non\_mineral\_value&       0.053***&      -0.356***&      -0.356***&       0.053***&      -0.044   &      -0.064   \\
            &     (0.006)   &     (0.076)   &     (0.107)   &     (0.019)   &     (0.098)   &     (0.132)   \\
\hline
F\_test\_     &               &      60.976   &      10.510   &               &      60.976   &      52.746   \\
\hline\hline
\multicolumn{7}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{7}{l}{\footnotesize * p<.1, ** p<.05, *** p<.01}\\
\end{tabular}
\end{table}


==> Results_a_.tex <==
\begin{table}[htbp]\centering
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Main Results}
\begin{tabular}{l*{6}{c}}
\hline\hline
            &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}\\
            &\multicolumn{1}{c}{number\_conflict}&\multicolumn{1}{c}{number\_conflict}&\multicolumn{1}{c}{number\_conflict}&\multicolumn{1}{c}{fatalities}&\multicolumn{1}{c}{fatalities}&\multicolumn{1}{c}{fatalities}\\
\hline
normalized\_mineral\_value&       0.007** &       0.059***&       0.059*  &       0.015   &      -0.078***&      -0.059   \\
            &     (0.003)   &     (0.012)   &     (0.033)   &     (0.017)   &     (0.015)   &     (0.048)   \\
[1em]
normalized\_non\_mineral\_value&       0.053***&      -0.356***&      -0.356***&       0.053***&      -0.044   &      -0.064   \\
            &     (0.006)   &     (0.076)   &     (0.107)   &     (0.019)   &     (0.098)   &     (0.132)   \\
\hline
F\_test\_     &               &      60.976   &      10.510   &               &      60.976   &      52.746   \\
\hline\hline
\multicolumn{7}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{7}{l}{\footnotesize * p<.1, ** p<.05, *** p<.01}\\
\end{tabular}
\end{table}


==> Table1_a.tex <==
\begin{table}[htbp]\centering
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Table 1}
\begin{tabular}{l*{1}{cccccc}}
\toprule
                    &         Sum&        Mean&          SD&         Min&         Max&           N\\
\midrule
(mean) incidence    &            &        0.89&        0.32&           0&           1&       1,252\\
(mean) number\_conflict&            &      184.41&      416.62&           1&       3,140&       1,109\\
(mean) fatalities   &            &      490.83&     1406.81&           0&      11,451&       1,109\\
\bottomrule
\end{tabular}
\end{table}


==> Table1_b.tex <==
\begin{table}[htbp]\centering
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Table 1}
\begin{tabular}{l*{1}{cccccc}}
\toprule
                    &         Sum&        Mean&          SD&         Min&         Max&           N\\
\midrule
(mean) incidence    &            &        0.96&        0.20&           0&           1&         628\\
(mean) number\_conflict&            &      223.13&      428.05&           1&       2,624&         602\\
(mean) fatalities   &            &      652.36&     1747.07&           0&      11,451&         602\\
\bottomrule
\end{tabular}
\end{table}


==> Table1_c.tex <==
\begin{table}[htbp]\centering
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Table 1}
\begin{tabular}{l*{1}{cccccc}}
\toprule
                    &         Sum&        Mean&          SD&         Min&         Max&           N\\
\midrule
(mean) incidence    &            &        0.81&        0.39&           0&           1&         624\\
(mean) number\_conflict&            &      138.44&      398.18&           1&       3,140&         507\\
(mean) fatalities   &            &      299.03&      800.33&           0&       6,138&         507\\
\bottomrule
\end{tabular}
\end{table}


==> Table1_d.tex <==
\begin{table}[htbp]\centering
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Table 1}
\begin{tabular}{l*{1}{cccccc}}
\toprule
                    &         Sum&        Mean&          SD&         Min&         Max&           N\\
\midrule
(mean) incidence    &            &        0.91&        0.28&           0&           1&      11,596\\
(mean) number\_conflict&            &      212.27&      415.84&           1&       3,140&      10,572\\
(mean) fatalities   &            &      446.75&     1332.44&           0&      11,451&      10,572\\
\bottomrule
\end{tabular}
\end{table}


==> Table1_e.tex <==
\begin{table}[htbp]\centering
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Table 1}
\begin{tabular}{l*{1}{cccccc}}
\toprule
                    &         Sum&        Mean&          SD&         Min&         Max&           N\\
\midrule
(mean) incidence    &            &        0.86&        0.35&           0&           1&      11,596\\
(mean) number\_conflict&            &      153.61&      384.84&           1&       3,140&       9,926\\
(mean) fatalities   &            &      491.84&     1370.53&           0&      11,451&       9,926\\
\bottomrule
\end{tabular}
\end{table}


==> Table2.tex <==
\begin{table}[htbp]\centering
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Table 2}
\begin{tabular}{l*{4}{c}}
\hline\hline
            &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}\\
            &\multicolumn{1}{c}{log\_number\_conflict}&\multicolumn{1}{c}{log\_number\_conflict}&\multicolumn{1}{c}{log\_fatalities}&\multicolumn{1}{c}{log\_fatalities}\\
\hline
log\_x\_mineral&       0.560** &       0.352** &       0.747***&       0.680***\\
            &     (0.257)   &     (0.159)   &     (0.279)   &     (0.234)   \\
\hline
F\_test\_     &      10.472   &      15.772   &      13.142   &      18.174   \\
\hline\hline
\multicolumn{5}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{5}{l}{\footnotesize * p<.1, ** p<.05, *** p<.01}\\
\end{tabular}
\end{table}


==> literature_review.tex <==
\begin{section}{Background}

Political theory has long been intrigued by the interplay between trade and conflict. In 1748, Montesquieu \citep{de1844esprit} offered an influential perspective on this question, positing that trade heightens the opportunity cost of war and therefore provides an incentive to minimize military conflicts. Conversely, a contrasting  ``realist view'' argues that increased economics rivalry between nations tends to intensify political tension \citep{copeland1996economic, thoenig2023trade}. \\



\noindent Economic theory soon overtook the topic and an extensive literature exists on the question. In 1980,  Montesquieu's theory has been explored in an economic model finding that mutual dependence established between two trading partners is sufficient to raise the costs of conflict, diminishing levels of dispute \citep{polachek1980conflict}. Later, \cite{martin2008civil} found that a pair of countries with more bilateral trade has lower probability of bilateral war. However, the authors argue that multilateral trade openness has the  opposite impact: countries that engage more importantly in global trade face a heightened likelihood of conflict. This arises because increased multilateral trade openness reduces their relative dependence with any specific bilateral partner, thereby lowering the opportunity cost of engaging in military hostilities. A large body of the literature also examines the impact of conflict on trade \citep{keshk2004trade, martin2008civil, martin2008make, glick2010collateral}, generally finding that conflicts are disruptive for trade. \cite{glick2010collateral} find that trade is substantially reduced not only between belligerent nations, where trade drops by 85\%, but also with nations that are not directly involved in the conflict in which trades decreases by 12\%. \\

\noindent On top of the political and classical economic theory perspectives on trade and war, the link between conflict and specific resources such as natural riches have been of particular interest in more recent empirical economics and policy debates. Indeed, conflicts play a prominent role amongst the several channels proposed to explain the concept of resource curse, which is a paradox that countries rich in non-renewable natural resources tend to display poor economic performance \citep{maystadt2014mineral, bruckner2012oil, ploeg2011natural}. Violence has been shown to respond to economic incentives created by mineral resource extraction \citep{berman2017mine, de2020origin}. Natural resources have also been found to extensively matter for organized crime \citep{buonanno2015poor}, homicide \citep{couttenier2017wild}, interstate war \citep{caselli2015geography} or mass killing of civilians \citep{esteban2015strategic}. The literature has also investigated specific commodities such as oil \citep{ross2006closer, lei2014giant, cotet2013oil}, which paves the way to more commodity-specific comparisons. This paper goes further in this direction analyzing different categories of minerals.     \\ 

\noindent The latest conflict happening at the border between East DRC and Rwanda is an example highlighting that this question is still highly relevant. Nicolas Kazadi, DRC’s finance minister, said in March 2023 that Rwanda exported close to one billion dollars in resources\footnote{Resources include gold, tin, tantalum, and tungsten} last year, even though the country has few mineral deposits of its own\footnote{\url{https://www.ft.com/content/ecf89818-949b-4de7-9e8a-89f119c23a69}}. In a region characterized by persistent instability where more than 6 million people died since 1996 due to repeated conflicts, and nearly 7 million individuals have been displaced internally, as reported by the United Nations\footnote{\url{https://www.france24.com/en/africa/20231030-record-6-9-million-internally-displaced-in-dr-congo-un-says}}, the abundance of natural resources—especially precious minerals—found in Congolese soil has spread the conflict in eastern DRC\footnote{\url{https://www.cfr.org/global-conflict-tracker/conflict/violence-democratic-republic-congo}}. \\ 



\noindent One important motivation of this paper lies behind the fact that use of mineral resources reached an unprecedented level and demand will probably continue growing in the coming decades \citep{vidal2021modelling}. Challenges regarding the adequacy of mineral resources in the context of population expansion and increasing standards of living have been a concern since the end of the 18th century, as highlighted in the work of  \cite{RePEc:hay:hetboo:malthus1798}. Even though research has shown that predictions of peak production due to resource exhaustion in the next 20–30 years are not necessarily correct \citep{meinert2016mineral}, the aim for a carbon neutral economy by 2050\footnote{\url{https://climate.ec.europa.eu/eu-action/climate-strategies-targets/2050-long-term-strategy_en}} comes with new challenges. Building new facilities such as wind turbines or solar power stations requires vast amounts of metals and other raw materials \citep{vidal2013metals}. This objective also comes with the promotion of new energy vehicles and it has been found that the rapid development of electric vehicles (EVs) contributed to a dramatic increase in in-use metal stocks from 0.7 kt in 2009 to 1.1 Mt in 2019 \citep{yang2021uncovering}. The higher scarcity and demand for mineral resources is consequently likely to intensify even further the so-called second wave of the scramble for Africa, potentially intensifying conflicts in the region.  \\

\noindent  This new scramble for Africa is different from the first one in many aspects. One of them is that due to globalization, different actors and not only Europe have economic and geopolitical interests in the region. Chinese firms notably invest heavily on the continent \citep{carmody2017new}, but Western powers and other emergent countries are also involved \citep{ayers2013beyond}. Nonetheless, there are some important similarities, especially because resources  were crucial in the first scramble for Africa \citep{carmody2017new}.  \\





\noindent As argued above, natural resources have been shown to considerably matter for conflict and more generally violence. Therefore, conducting comprehensive measurements to determine the impact of mineral trade on conflict, as well as identifying which type of minerals is most pertinent to explain such a relationship, holds considerable importance from both short-term and long-term perspectives. This is particularly crucial in light of the imminent challenges posed by climate change. 







\end{section}
